Exploiting Scaling Constants to Facilitate the Convergence of Indirect Trajectory Optimization Methods

This note develops easily applicable techniques that improve the convergence and reduce the computational time of indirect low thrust trajectory optimization when solving fuel- and time-optimal problems. For solving fuel optimal (FO) problems, a positive scaling factor -- $\Gamma_{TR}$ -- is introduced based on the energy optimal (EO) solution to establish a convenient profile for the switching function of the FO problem. This negates the need for random guesses to initialize the indirect optimization process. Similarly, another scaling factor-$\beta$-, is introduced when solving the time-optimal (TO) problem to connect the EO problem to the TO. The developed methodology for the TO problem was crucial for the GTOC11 competition. Case studies are conducted to validate the solution process in both TO and FO problems. For geocentric cases, the effect of eclipses and $J_2$ perturbations were also considered. The examples show that EO can provide a good guess for TO and FO problems and that introducing the constants can reduce the initial residuals and improve convergence. It is also shown that the equation for the Lagrangian multiplier of mass and the associated boundary condition can be ignored for both FO and TO cases without affecting optimality. This simplification reduces the problem dimensions and improves efficiency.

==> images/lambdanonzero.tex <==
\section{Fuel Optimal Problem}

\subsection{Optimization Problem Formulation}
\subsubsection{The Energy Optimal Problem}
In this method, the energy optimal problem is formulated to minimize: 
\begin{equation}
    J = \frac{1}{2}\frac{T_{max}}{I_{sp} g_0}  \int^{t_f}_{t0} \tau_e^2 dt 
    \label{3}
\end{equation}

subject to the spacecraft dynamics defined in the previous section. Here, $t_f$ and $t_0$ denotes the start and end times of the mission respectively. $\tau_e$ denotes the energy optimal thrust ratio.  The terminal constraints that must hold are given in Equation \ref{conditions2}. \par
\begin{equation}\label{conditions2}
\boldsymbol{x}(t_0) = \boldsymbol{x_0}, \  \boldsymbol{x}(t_f) = \boldsymbol{x_f}, \  m(t_0) = m_0,  \ m(t_f) = free, \ \lambda_m(t_f) = 0,
\end{equation} 

  \subsubsection{The Fuel Optimal Problem}
The fuel optimal problem entails minimizing: 
\begin{equation}\label{lambdanonzerofopt2}
    J = \tau_{TR}\frac{T_{max}}{I_{sp} g_0}\int^{t_f}_{t0} \tau_f  \ dt 
\end{equation}

Here, $t_f$ and $t_0$ denotes the start and end times of the mission respectively. $\tau_{TR}$ is a constant that is obtained by solving the energy optimal problem described above. The terminal constraints that must hold are same as those given in Equation \ref{conditions2}.
 
 
 

\subsection{Solution methodology}
As mentioned, a homotopic approach is utilized to solve the energy optimal problem. Thus, the energy optimal problem is linearized and analytically solved first. Then this solution is used as an initial guess for solving the nonlinear energy optimal problem.


\subsubsection{Linear energy optimal problem }
Linearizing the spacecraft dynamics with respect to a point in the unperturbed motion of the spacecraft given by $x_n$, we can obtain the following. Note that the subscript $el$ indicates that the quantity is specific to the linear energy optimal problem.
\begin{equation}
    \dot{\boldsymbol{x}}=\boldsymbol{C}\left(\boldsymbol{x}_{n}, t\right) \boldsymbol{x}+\frac{T_{max}}{m} \boldsymbol{B}\left(\boldsymbol{x}_{n}, t\right) \tau_{el} \hat{\boldsymbol{\alpha}_{el}}+\boldsymbol{D}\left(\boldsymbol{x}_{n}, t\right), \quad \boldsymbol{x}\left(t_{0}\right)=\boldsymbol{x}_{0}
\end{equation}
where: 
\begin{equation}
    \begin{gathered}
\boldsymbol{C}\left(\boldsymbol{x_{n}}, t\right) \triangleq \partial \boldsymbol{A}(\boldsymbol{x}, t) /\left.\partial \boldsymbol{x}\right|_{\boldsymbol{x}=\boldsymbol{x_{n}}} \\
\boldsymbol{D}\left(\boldsymbol{x_{n}}, t\right) \triangleq \boldsymbol{A}\left(\boldsymbol{x_{n}}, t\right)-\boldsymbol{C}\left(\boldsymbol{x_{n}}, t\right) \boldsymbol{x_{n}}
\end{gathered}
\end{equation}

Here, $ \boldsymbol{x}(t) = \boldsymbol{x}_{actual}(t) - \boldsymbol{x}_n(t)$, which is the the deviation of the orbital elements from the reference trajectory.\par 
Upon linearization of the energy optimal problem, the objective function remains the same as Equation \ref{4}. The analytical solution to the linear energy optimal problem is obtained using the methodology described in \cite{Altitude-dependent2010c}, with a minor change to the $\Phi$ matrix due to the differences in problem dynamics. Hence: 
\begin{equation}
    \Phi = \left[\begin{array}{cc}
\boldsymbol{C} & -\frac{T_{\max } I_{sp}g_0}{m^{2} } \boldsymbol{B} \boldsymbol{B}^{T} \\
\boldsymbol{0} & -\boldsymbol{C}^{T}
\end{array}\right]
\end{equation}

\subsubsection{Nonlinear Energy Optimal Problem}
 
The energy optimal problem given in \ref{3} can be transformed into a two point boundary value problem (TPBVP) using Pontryagin’s maximum principle. By introducing the costate vector  $\boldsymbol{\lambda_x} = [\lambda_p, \lambda_f, \lambda_g, \lambda_h, \lambda_k, \lambda_L]^T$, the Hamiltonian of the energy optimal problem can be constructed as follows.
\begin{equation}
     \mathcal{H} =  \boldsymbol{\lambda_x}^T[ \boldsymbol{A} +\frac{T_{\max }}{m} \boldsymbol{B} \tau_e \hat{\boldsymbol{\alpha}}_e] +  \frac{1}{2}\frac{T_{max}}{I_{sp} g_0}  \tau_e^2
\end{equation}

In this case, the thrust magnitude and direction that minimizes the Hamiltonian are: 
\begin{equation}
   \hat{\boldsymbol{\alpha}}_e^* = \frac{- \boldsymbol{B}^T \boldsymbol{\lambda_x}}{|\boldsymbol{B}^T \boldsymbol{\lambda_x}| } \ \text{and} \  \tau_e^* = \frac{I_{sp} g_0}{m} |\boldsymbol{B}^T \boldsymbol{\lambda_x}| 
\end{equation}

Substituting $\hat{\boldsymbol{\alpha}}_e^*$ and $ \tau_e^*$ we can rewrite the dynamics and the Euler-Lagrange equations and derive the time derivatives of the costates as follows. 
\begin{equation}\label{xdot}
    \boldsymbol{\dot{x}} = \boldsymbol{A}  - \frac{T_{max}I_{sp}g_0}{m^2}\boldsymbol{B}\boldsymbol{B}^T \boldsymbol{\lambda_x}
\end{equation}
% \begin{equation}\label{ldot}
%      \boldsymbol{\lambda_x} = -\frac{\partial{ \mathcal{H}}}{\partial{ \boldsymbol{x}}} \approx -\frac{\partial{ A}}{\partial{ \boldsymbol{x}}}^T
%      \boldsymbol{\lambda_x} 
% \end{equation}


\begin{equation}\label{ldot}
     \boldsymbol{\dot{\lambda}_x} = -\frac{\partial{ \mathcal{H}}}{\partial{ \boldsymbol{x}}} = -(\frac{\partial{ \boldsymbol{A}}}{\partial{ \boldsymbol{x}}} -
     \frac{T_{max} I_{sp} g_0}{m^2}|\boldsymbol{B}^T \boldsymbol{\lambda_x}|\frac{\partial{ \boldsymbol{B}}} {\partial{ \boldsymbol{x}}}   )^T
     \boldsymbol{\lambda_x} 
\end{equation}

The costate dynamics are further simplified by assuming  $  \boldsymbol{\dot{\lambda}_x}   \approx -\frac{\partial{\boldsymbol{A}}}{\partial{ \boldsymbol{x}}}^T \boldsymbol{\lambda_x}$ and $\dot{m} = 0$.
Finally, the optimal control problem yeilds a TPBVP of the following form: 
\begin{equation}
    \boldsymbol{\Phi}(\boldsymbol{\lambda_{x}}(t_0)) = [\boldsymbol{x}(t_0) - \boldsymbol{x_0}, \boldsymbol{x}(t_f) - \boldsymbol{x_f}] = \boldsymbol{0}
\end{equation}

This system can then be solved using a nonlinear solver under the boundary conditions given in Eq. \ref{conditions2}. The initial guess required for this process is obtained from the linear energy optimal problem.  \par 
\paragraph{Reintroduction of variable mass to the energy optimal problem}
 While assuming constant mass permits ease of computation, it is not an accurate assumption. Hence, the mass variation is reintroduced to the energy optimal solution prior to using it as an initial guess for the fuel optimal problem. This is done by separately integrating the spacecraft mass using ode45, where $ \dot{m} = -\frac{T_{max} \tau_e}{I_{sp}}$.
 

\subsubsection{Fuel Optimal Problem}

The fuel optimal problem given in Equation \ref{lambdanonzerofopt2} can be transformed into a two point boundary value problem (TPBVP) using Pontryagin’s maximum principle. First, the Hamiltonian of this problem is built as follows.
\begin{equation}
     \mathcal{H} =  \boldsymbol{\lambda_x}^T[ \boldsymbol{A} +\frac{T_{\max }}{m} \boldsymbol{B} \tau_f \hat{\boldsymbol{\alpha}}_f] +  \tau_{TR}\frac{T_{max}}{I_{sp} g_0}  \tau_f - \lambda_m \frac{T_{max}}{I_{s p} g_{0}} \tau_f
\end{equation}

The optimal thrust direction that minimizes the Hamiltonian is: 
\begin{equation}
    \hat{\boldsymbol{\alpha}}_f^* = \frac{- \boldsymbol{B^T \lambda_x}}{| \boldsymbol{B^T \lambda_x}|} = \hat{\boldsymbol{\alpha}}_e^* 
\end{equation}

Substituting $\hat{ \boldsymbol{\alpha}}_f^*$ to the Hamiltonian:  
$$ \mathcal{H} = \boldsymbol{\lambda_x}^T\boldsymbol{A} + \tau_f^* \frac{T_{max}}{I_{sp}g_0} (\tau_{TR} - \frac{I_{sp} g_0}{m}|\boldsymbol{B}^T \boldsymbol{\lambda_x}| - \lambda_m) = \boldsymbol{\lambda_x}^T\boldsymbol{A} + \tau_f^* \frac{T_{max}}{I_{sp}g_0}(\tau_{TR} - \tau_e^* - \lambda_m)$$



Hence, to minimize the Hamiltonian the thrust ratio must be defined as: 
\begin{equation}\label{fopt2}
\begin{aligned}
\tau_{TR} -\tau_e^* - \lambda_m  > 0 &\Rightarrow \tau_f^* = 0   \ \text{and} \ 
\tau_{TR} -\tau_e^* - \lambda_m  < 0 &\Rightarrow \tau_f^* = 1   \\
     \end{aligned}
\end{equation}

This shows how the control of the fuel optimal is tied to the control of the energy optimal solution through $\tau_{TR}$. Now, $\tau_f^*$ can be formulated as follows, where $\rho$ represents a switching function. 
\begin{equation}
    \tau_f^* = \frac{1}{2}(1- \text{sgn}(\rho)) \ \text{where}  \ \rho = (\tau_{TR} - \tau_e^* - \lambda_m)
\end{equation}

 

The costate differential equations (Euler–Lagrange equations) can then be obtained as: 

\begin{align}
\boldsymbol{\dot{\lambda_x}} &= -\frac{\partial{\mathcal{H}  }}{\partial{ \boldsymbol{x}}} = -(\frac{\partial{ A}}{\partial{ \boldsymbol{x}}} + \frac{T_{\max }}{m}\frac{\partial\boldsymbol{B}}{\partial \boldsymbol{x}} \tau_f \hat{\boldsymbol{\alpha}}_f)^T
     \boldsymbol{\lambda_x} \\
     \dot{\lambda_m} &= -\frac{\partial{ \mathcal{H}}}{\partial{ {m}}} =-\frac{T_{\max } \tau_f}{m^{2}}|\boldsymbol{B \lambda_{x}}|
\end{align}


Substituting $\hat{\boldsymbol{\alpha}}_f*$ and $ \tau_f^*$ we can rewrite the dynamics and the Euler-Lagrange equations of the problem as follows.

\begin{equation}
\begin{aligned}\label{fopt}
        &\dot{ \boldsymbol{x}}= \boldsymbol{A}( \boldsymbol{x}, t)-\frac{T_{max}}{2m} (1- \text{sgn}(\rho)) \frac{\boldsymbol{B B^T \lambda_x}}{| \boldsymbol{B^T \lambda_x}|}  \\
&\dot{m}=\frac{-T_{max}}{2I_{s p} g_{0}} (1- \text{sgn}(\rho))\\
&\dot{ \boldsymbol{\lambda_x}} = -(\frac{\partial{  \boldsymbol{A}}}{\partial{ \boldsymbol{x}}} -
     \frac{T_{max}}{2m_0}\frac{\partial{ \boldsymbol{B}}}{\partial{ \boldsymbol{x}}} (1- \text{sgn}(\rho)) \frac{\boldsymbol{B^T \lambda_x}}{| \boldsymbol{B^T \lambda_x}|}  )^T
     \boldsymbol{\lambda_x} \\
     &\dot{\lambda_m} = -\frac{T_{\max } (1- \text{sgn}(\rho))}{2m^{2}}|\boldsymbol{B \lambda_{x}}|
     \end{aligned}
\end{equation}


Equations \ref{fopt} can be  simplified to  Equations \ref{sfopt}, which have less computational cost and complexity.  Equations \ref{fopt} shall be referred to as the full fuel optimal dynamics, while Equations \ref{sfopt} shall be called the simplified fuel optimal  dynamics from here on.  Both are used in the solution generation process.



\begin{equation}
\begin{aligned}\label{sfopt}
        &\dot{ \boldsymbol{x}}= \boldsymbol{A}( \boldsymbol{x}, t)-\frac{T_{max}}{2m} (1- \text{sgn}(\rho)) \frac{\boldsymbol{B B^T \lambda_x}}{| \boldsymbol{B^T \lambda_x}|}  \\
&\dot{m}=\frac{-T_{max}}{2I_{s p} g_{0}} (1- \text{sgn}(\rho))\\
&\dot{ \boldsymbol{\lambda_x}} \approx -(\frac{\partial{  \boldsymbol{A}}}{\partial{ \boldsymbol{x}}})^T
     \boldsymbol{\lambda_x} \\
&\dot{\lambda_m} = 0
     \end{aligned}
\end{equation}
Note that in Equations \ref{sfopt}, the mass costate derivative is assumed to be zero by assuming the mass to be constant in the Hamiltonian. The initial and final states must satisfy Equation \ref{conditions2}. Thus, the problem now consists of finding the initial lagrangian multipliers that satisfy the following shooting function.
\begin{equation}
    \boldsymbol{\Phi}(\boldsymbol{\lambda_{x}}(t_0)) = [\boldsymbol{x}(t_0) - \boldsymbol{x_0}, \boldsymbol{x}(t_f) - \boldsymbol{x_f}, \lambda_m (t_f)] = \boldsymbol{0}
\end{equation}
The initial guess required for solving this shooting function is obtained from the energy optimal problem. 



 Hamiltonian. 
\paragraph{Determination of $\tau_{TR}$} Prior to solving the fuel optimal shooting problem $\tau_{TR}$ must be determined. According to Equation \ref{fopt2}, provided that $\tau_{TR}$ is set correctly, the energy optimal thrust profile can be discretised into the fuel optimal thrust profile for a given trajectory. In this paper, we propose setting $\tau_{TR}$ such that the continous and discreetised thrust profile of the energy optimal solution has the same $\Delta v$ contribution. Hence, the steps taken to calculate $\tau_{TR}$ are : 
\begin{enumerate}
    \item Obtain the optimal nonlinear energy solution and its thrust profile ($\tau_e(t)$).
    \item Calculate the total thrust over time as $T = \int^{t_f}_{t0} \tau_e(t) \ dt$
    \item Let $TR_L = 0$ and $TR_R = \max(\tau_e(t))$, set ${T_{total}} = 0$. 
    \item While $abs(T_{total} - T) > 0 $:
    \begin{enumerate}
        \item Calculate $\tau_{TR} = \frac{TR_L + TR_R}{2}$
        \item Construct a discreet, bang bang thrust profile ($\tau_{discreet}(t)$) from the continuous $\tau_e(t)$, such that: 
    \begin{equation}
\begin{aligned}
    \text{If} \ \tau_e(t)&> \tau_{TR} \ \rightarrow \ \tau_{discreet}(t)  = \frac{1}{ \frac{m_(t)}{m_0}} \\ 
    \text{If} \ \tau_e(t) &< \tau_{TR}\ \rightarrow \ \tau_{discreet}(t) = 0
    \end{aligned}
    \end{equation}
    \item Calculate the thrust over time for $\tau_{discreet}(t)$ as $T_{total} = \int^{t_f}_{t0} \tau_{discreet}(t) \ dt $

    \item If $T_{total} > T \rightarrow TR_L = \tau_{TR}$ and if $T_{total} < T \rightarrow TR_R = \tau_{TR}$
    \end{enumerate}
    
    \item Return $\tau_{TR}$.
    \end{enumerate}
    
\paragraph{Continuation Strategy}
In practice, going directly from a continuous thrust ratio solution (Energy optimal) to a discreet $\tau_f$ solution (Fuel optimal) may cause convergence issues. Hence we can introduce a continuation parameter k to the expression for $\tau_f^*$, such that k can be slowly increased from 0 to 1 to make $\tau_f$ increasingly discreet step by step. Hence $\tau_f^*$ is actually defined as follows: 
\begin{equation}
    \tau_f^* = \frac{1}{2} - \frac{1}{2}\tanh \left({\frac{\tau_{TR}  - \tau_e^*}{1- k}}\right)
\end{equation}

\subsection{Case Study}

In this section, a low thrust fuel optimal trajectory is designed from Earth to the Asteroid Tempel 1,first with the simplified dynamics (Equations \ref{sfopt}) and then using the full fuel optimal dynamics (Equations \ref{sfopt}). The accuracy of the solutions and the computational time is compared with each other. 

The problem parameters are shown in Table \ref{testcasepara} and are same as those given in \cite{Altitude-dependent2010c}.

\begin{table}[hbt!]
\centering 
\caption{Parameters for Earth to Tempel 1 mission}
\begin{tabular}{l c}
 \hline
Specific impulse,s   & 1300                    \\ 
Maximum thrust , N             & 0.60                    \\ 
Initial mass, kg              & 1000                    \\ 
Launch time, TDB    & 9 Aug. 2015, 00:00:00.0 \\ 
Time of flight, days & 420                     \\ \hline
\end{tabular}
\label{testcasepara}
\end{table}

\subsubsection{Solution with the Simplified Dynamics}
Table \ref{costatesinit1} lists the variation of initial costates going from the energy optimal to the fuel optimal solution. The total CPU time spent on generating this solution on C++ is 165.2 ms. The switched method described in \cite{Altitude-dependent2010c} takes 233.9 ms to derive the same optimal solution. 
\begin{table}[hbt!]
\centering 
\caption{Initial costates obtained at each step of the solution for the Earth to Tempel 1 trajectory}
\begin{tabular}{lcccccc}
\hline
~ & $\lambda_p ({m/s^3})$ & $\lambda_f({m^2/s^3})$ & $\lambda_g({m^2/s^3})$  & $\lambda_h({m^2/s^3})$  & $\lambda_k({m^2/s^3})$  & $\lambda_L({m^2/s^3})$ \\
\hline 
Energy optimal & 0.0895                & -0.2478                & -0.0633                & -0.2080                & -0.8123                & -0.0801                \\
k = 0          & 0.0330                & -0.1026                & -0.0243                & -0.1453                & -0.4703                & -0.0302                \\
k = 0.2        & 0.0228                & -0.0951                & -0.0245                & -0.1383                & -0.4696                & -0.0277                \\
k = 0.4        & 0.0083                & -0.0879                & -0.0258                & -0.1299                & -0.4756                & -0.0247                \\
k = 0.6        & -0.0157               & -0.0815                & -0.0282                & -0.1163                & -0.4876                & -0.0207                \\
k = 0.8        & -0.0594               & -0.0743                & -0.030                 & -0.0868                & -0.4931                & -0.0143                \\
k = 0.99       & -0.1448               & -0.0526                & -0.0013                & -0.0090                & -0.4710                & -0.001    \\ \hline             
\end{tabular}
\label{costatesinit1}
\end{table}



\begin{figure}[hbt!]
    \centering
    \includegraphics[width = 0.7\textwidth]{images/masstau1.png}
    \caption{Profile of mass at each step of the solution process (top) and the profile of the optimal thrust ratio $\tau$ at each step of the solution process ($\tau_{TR} = 0.41083$) (bottom)}
    \label{mass1}
\end{figure}


Figures \ref{mass1} illustrates the profiles of thrust ratio and mass of the spacecraft. The bang bang control structure that contains two coast arcs and three burning arcs are obtained for the fuel optimal trajectory. The total propellant consumption of the mission is 349.35 kg, which is comparable to the 348.26 kg observed in \cite{Altitude-dependent2010c} .  


To illustrate the effectivity of the thresholding method, the switching function ($\rho$) and the thrust ratio ($\tau$) are plotted against time (Figure \ref{switching}), for the Earth to Tempel 1 test case. 
$\text{TR} = 0.41564$ is the case where the value of TR has been obtained from the thresholding method described. 

\begin{figure}[hbt!]
    \centering
    \includegraphics[width = 0.5\textwidth]{images/rhoswitch.png}
    \caption{Profiles of the switching function and thrust ratio for Earth to Tempel 1 test case}
    \label{switching}
\end{figure}

It can be seen that the profile of $\rho$ generated with the TR value obtained from the thresholding method matches very closely to the $\rho$ profile of the final fuel optimal solution. In general TR is set to be unity in most circumstances, and it can be seen that the switching function profile for $\text{TR} = 1$ varies strongly from the finale fuel optimal solution, indicating that the thresholding does indeed provide a better initial guess for the fuel optimal problem. 
Similarly, it can be seen that the TR value generated from the thresholding method has a $\tau$ profile that matches very closely with the final fuel optimal solution obtained.




\subsubsection{Solution with Full Dynamics}

Table \ref{costatesinit2} lists the variation of initial costates going from the Energy optimal to the fuel optimal solution. The total CPU time spent on generating this solution on C++ is 205.3 ms. Once again the computational time is less compared to the 233.9 ms taken by the Warm Start method \cite{Altitude-dependent2010c}, but higher compared to the solution with simplified dynamics. 

\begin{table}[hbt!]
\centering 
\caption{Initial costates obtained at each step of the solution for the Earth to Tempel 1 trajectory}
\begin{tabular}{lccccccl}
\hline
~ & $\lambda_p ({kg/m})$ & $\lambda_f({kg})$ & $\lambda_g({kg})$  & $\lambda_h({kg})$  & $\lambda_k({kg})$  & $\lambda_L({kg})$ & $\lambda_m({m/s/kg})$ \\
\hline 
Energy optimal & 0.1189                & -0.1800                & -0.1124                & -0.3319                & -0.7352                & -0.0836                & 0.0                    \\
k = 0          & 0.0606                & -0.0772                & -0.0288                & -0.1308                & -0.2976                & -0.0372                & 0.2342                 \\
k = 0.2        & 0.0552                & -0.0728                & -0.0291                & -0.1280                & -0.2898                & -0.0352                & 0.2224                 \\
k = 0.4        & 0.0489                & -0.0685                & -0.0308                & -0.1266                & -0.2850                & -0.0332                & 0.2109                 \\
k = 0.6        & 0.0400                & -0.0645                & -0.0356                & -0.1278                & -0.2852                & -0.0310                & 0.1999                 \\
k = 0.8        & 0.0200                & -0.0610                & -0.0481                & -0.1328                & -0.2889                & -0.0280                & 0.1895                 \\
k = 0.99       & -0.0767               & -0.0292                & -0.0348                & -0.1257                & -0.2342                & -0.0115                & 0.1706                
    \\ \hline
\end{tabular}
\label{costatesinit2}
\end{table}


\begin{figure}[hbt!]
    \centering
    \includegraphics[width = 0.7\textwidth]{images/masstau2.png}
    \caption{Profile of mass at each step of the solution process (top) and the profile of the optimal thrust ratio $\tau$ at each step of the solution process ($\tau_{TR} = 0.3958$) (bottom)}
    \label{mass2}
\end{figure}



Figures \ref{mass2} illustrate the profiles of thrust ratio and mass of the spacecraft. The bang bang control structure that constains two coast arcs and three burning arcs are obtained for the fuel optimal trajectory. The total propellant consumption of the mission is 348.88 kg, which is comparable to the 348.26 kg observed in \cite{Altitude-dependent2010c} .  


